Octopus: Alleviating Hallucination via Dynamic Contrastive Decoding

Large Vision-Language Models (LVLMs) have obtained impressive performance in visual content understanding and multi-modal reasoning. Unfortunately, these large models suffer from serious hallucination problems and tend to generate fabricated responses. Recently, several Contrastive Decoding (CD) strategies have been proposed to alleviate hallucination by introducing disturbed inputs. Although great progress has been made, these CD strategies mostly apply a one-size-fits-all approach for all input conditions. In this paper, we revisit this process through extensive experiments. Related results show that hallucination causes are hybrid and each generative step faces a unique hallucination challenge. Leveraging these meaningful insights, we introduce a simple yet effective Octopus-like framework that enables the model to adaptively identify hallucination types and create a dynamic CD workflow. Our Octopus framework not only outperforms existing methods across four benchmarks but also demonstrates excellent deployability and expansibility. Code is available at https://github.com/LijunZhang01/Octopus.

==> no_use_fig_table/table2_01.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
\caption{xxx.}
\begin{tabular}{lcccccccc}\toprule
 &\multicolumn{8}{c}{POPE\_MSCOCO} \\ 
 &\multicolumn{2}{c}{Random}&\multicolumn{2}{c}{Popular}&\multicolumn{2}{c}{Adversarial}&\multicolumn{2}{c}{ALL}  \\
 &Accuracy &F1 &Accuracy &F1 &Accuracy &F1 &Accuracy &F1\\
 \midrule
  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  LLaVA-1.5& 83.77  & 81.94  & 82.57  & 80.86  & 79.77  & 78.47  & 82.04  & 80.42 \\
  LLaVA-1.5+VCD& 85.43  & 83.99  & 82.07  & 80.35  & 80.27  & 79.49  & 82.59  & 81.28 \\
  LLaVA-1.5+M3ID& 86.13  & 81.85  & 83.17  & 80.77  & 79.50  & 78.15  & 82.93  & 80.26 \\
  LLaVA-1.5+AVISC& 83.80  & 82.04  & 80.90  & 81.27  & 79.63  & 78.42  & 81.44  & 80.58  \\
  LLaVA-1.5+Octopus& \textbf{86.53}  & \textbf{85.11  }  & \textbf{84.60}  & \textbf{83.20}  & \textbf{81.60}  & \textbf{80.52}  & \textbf{84.24}  & \textbf{82.94} \\
  \midrule
  InstructBLIP& 81.53  & 81.19  & 78.47  & 78.75  & 77.43  & 78.00  & 79.14  & 79.31 \\
  InstructBLIP+VCD& 82.03  & 81.56  & 79.13  & 79.20  & 77.23  & 77.72  & 79.46  & 79.49 \\
  InstructBLIP+M3ID& 82.33  & 81.53  & 80.90  & 80.42  & 78.53  & 78.49  & 80.59  & 80.15 \\
  InstructBLIP+AVISC& 86.03  & 84.41  & 84.27  & 82.77  & 81.83  & 80.67  & 84.04  & 82.62 \\
  InstructBLIP+Octopus& \textbf{86.63}  & \textbf{85.30}  & \textbf{84.90}  & \textbf{83.55}  & \textbf{82.83}  & \textbf{81.43}  & \textbf{84.79}  & \textbf{83.43} \\


% \midrule
% \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% \midrule
\bottomrule
\end{tabular}

\label{tab:table2}
\end{table*}


==> no_use_fig_table/table_2.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
\caption{xxx.}
\begin{tabular}{ccccccccccc}\toprule
 \multirow{2}*{Dataset}&\multirow{2}*{Setup} &\multirow{2}*{Method}  &\multicolumn{4}{c}{LLaVA 1.5} &\multicolumn{4}{c}{InstructBLIP} \\ \cmidrule(lr){4-7} \cmidrule(lr){8-11}
 & & &Accuracy &Precision &Recall &F1 &Accuracy &Precision &Recall &F1\\
 \midrule
  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  \multirow{15}*{MSCOCO}& \multirow{5}*{Random}&base& 83.77  & 92.31  & 73.67  & 81.94  & 81.53  & 82.71  & \textbf{79.73}  & 81.19 \\
  & &VCD& 85.43  & 93.25  & 76.40  & 83.99  & 82.03  & 83.77  & 79.47  & 81.56 \\
  & &M3ID& 86.13  & 92.59  & 73.33  & 81.85  & 82.33  & 85.40  & 78.00  & 81.53 \\
  & &AVISC& 83.80  & 92.04  & 74.00  & 82.04  & 86.03  & \textbf{95.53}  & 75.60  & 84.41 \\
  & &Octopus& \textbf{86.53}  & \textbf{95.14}  & \textbf{77.00}  & \textbf{85.11}  & \textbf{86.63}  & 94.78  & 75.53  & \textbf{85.30} \\
\cline{2-11}
  & \multirow{5}*{Popular}&base& 82.57  & 89.62  & 73.67  & 80.86  & 78.47  & 77.73  & \textbf{79.80}  & 78.75  \\
  & &VCD& 82.07  & 88.86  & 73.33  & 80.35  & 79.13  & 78.94  & 79.47  & 79.20 \\
  & &M3ID& 83.17  & 81.34  & \textbf{80.20}  & 80.77  & 80.90  & 82.48  & 78.47  & 80.42 \\
  & &AVISC& 80.90  & \textbf{95.25}  & 70.87  & 81.27  & 84.27  & 91.45  & 75.60  & 82.77 \\
  & &Octopus& \textbf{84.60}  & 91.52  & 76.27  & \textbf{83.20}  & \textbf{84.90}  & \textbf{91.78}  & 76.67  & \textbf{83.55} \\
\cline{2-11}
  & \multirow{5}*{Adversarial}&base& 79.77  & 83.85  & 73.73  & 78.47  & 77.43  & 76.09  & \textbf{80.00}  & 78.00 \\
  & &VCD& 80.27  & 82.76  & 76.47  & 79.49  & 77.23  & 76.10  & 79.40  & 77.72 \\
  & &M3ID& 79.50  & 83.65  & 73.33  & 78.15  & 78.53  & 78.65  & 78.33  & 78.49 \\
  & &AVISC& 79.63  & 83.40  & 74.00  & 78.42  & 81.83  & 86.20  & 75.80  & 80.67 \\
  & &Octopus& \textbf{81.60}  & \textbf{85.53}  & \textbf{76.01}  & \textbf{80.52}  & \textbf{82.83}  & \textbf{88.69}  & 75.27  & \textbf{81.43} \\
\midrule
  \multirow{15}*{A-OKVQA}& \multirow{5}*{Random}&base& 84.93  & 89.16  & 79.53  & 84.07  & 81.33  & 78.52  & 86.27  & 82.21 \\
  & &VCD& 85.53  & 87.64  & 82.73  & 85.12  & 81.57  & 78.78  & \textbf{86.40}  & 82.42 \\
  & &M3ID& 85.06  & 88.85  & 80.20  & 84.30  & 82.37  & 81.18  & 84.27  & 82.70 \\
  & &AVISC& 87.33  & \textbf{95.09}  & 78.73  & 86.14  & 87.10  & \textbf{89.95}  & 83.53  & 86.62 \\
  & &Octopus& \textbf{88.57}  & 92.26  & \textbf{84.20}  & \textbf{88.05}  & \textbf{87.43}  & 89.24  & 85.13  & \textbf{87.14}  \\
\cline{2-11}
  & \multirow{5}*{Popular}&base& 80.90  & 81.77  & 79.53  & 80.64  & 76.87  & 72.69  & 86.07  & 78.82 \\
  & &VCD& 79.67  & 79.83  & 79.40  & 79.61  & 77.30  & 73.10  & \textbf{86.40}  & 79.19 \\
  & &M3ID& 80.90  & 81.33  & 80.20  & 80.77  & 78.33  & 75.33  & 84.27  & 79.55 \\
  & &AVISC& 85.03  & \textbf{90.08}  & 78.73  & 84.03  & 82.47  & 81.79  & 83.53  & 82.65 \\
  & &Octopus& \textbf{85.33}  & 86.15  & \textbf{84.20}  & \textbf{85.17}  & \textbf{83.20}  & \textbf{82.30}  & 83.91  & \textbf{83.10} \\
\cline{2-11}
  & \multirow{5}*{Adversarial}&base& 74.80  & 72.63  & 79.60  & 75.59  & 71.40  & 66.67  & \textbf{85.60}  & 74.96  \\
  & &VCD& 75.03  & 71.87  & 82.27  & 76.72  & 72.47  & 67.39  & 87.07  & 75.97 \\
  & &M3ID& 74.80  & 72.28  & 80.47  & 76.15  & 72.07  & 67.95  & 83.53  & 74.94  \\
  & &AVISC& \textbf{79.27}  & \textbf{79.58}  & 78.73  & 79.16  & 76.47  & 73.16  & 83.60  & 78.03 \\
  & &Octopus& 78.50  & 75.74  & \textbf{84.87}  & \textbf{79.60}  & \textbf{77.20}  & \textbf{74.21}  & 84.10  & \textbf{78.85} \\
\midrule
  \multirow{15}*{GQA}& \multirow{5}*{Random}&base& 84.80  & 87.88  & 80.73  & 84.16  & 80.57  & 77.47  & 86.20  & 81.60 \\
  & &VCD& 85.63  & 86.89  & 83.93  & 85.38  & 81.73  & 79.20  & \textbf{86.40}  & 82.55 \\
  & &M3ID& 84.80  & 87.50  & 81.20  & 84.23  & 81.17  & 79.87  & 83.33  & 81.57 \\
  & &AVISC& 87.40  & \textbf{95.17}  & 78.80  & 86.21  & 85.30  & 88.57  & 81.07  & 84.65 \\
  & &Octopus& \textbf{88.23}  & 91.41  & \textbf{84.40}  & \textbf{87.76}  & \textbf{85.37}  & \textbf{86.11}  & 84.33  & \textbf{85.21} \\
\cline{2-11}
  & \multirow{5}*{Popular}&base& 79.37  & 78.59  & 80.73  & 79.64  & 74.67  & 70.17  & 85.80  & 77.20 \\
  & &VCD& 78.73  & 76.03  & 83.93  & 79.78  & 74.63  & 69.94  & \textbf{86.40}  & 77.30 \\
  & &M3ID& 79.23  & 78.13  & 81.20  & 79.63  & 75.77  & 72.33  & 83.47  & 77.50 \\
  & &AVISC& \textbf{83.33}  & \textbf{86.66}  & 78.80  & 82.54  & 80.63  & 80.37  & 81.07  & 80.72\\
  & &Octopus& 83.00  & 82.10  & \textbf{84.40}  & \textbf{83.23}  & \textbf{81.03}  & \textbf{80.33}  & 82.20  & \textbf{81.25} \\
\cline{2-11}
  & \multirow{5}*{Adversarial}&base& 76.00  & 74.13  & 79.87  & 76.89  & 72.63  & 67.78  & \textbf{86.27}  & 75.92 \\
  & &VCD& 76.40  & 72.76  & 84.40  & 78.15  & 71.93  & 67.21  & 85.67  & 75.32 \\
  & &M3ID& 75.83  & 73.58  & 80.60  & 76.93  & 73.47  & 69.47  & 83.73  & 75.94 \\
  & &AVISC& \textbf{80.37}  & \textbf{81.52}  & 78.53  & 80.00  & 77.60  & 75.91  & 80.87  & 78.31  \\
  & &Octopus& 80.23  & 77.60  & \textbf{85.00}  & \textbf{81.13}  & \textbf{78.37}  & \textbf{77.19}  & 80.53  & \textbf{78.83}  \\
% \midrule
% \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% \midrule
\bottomrule
\end{tabular}

\label{tab:table2}
\end{table*}


==> no_use_fig_table/table_3.tex <==
% \begin{table*}[t]
% \centering
% \small
% % \setlength{\tabcolsep}{2.5pt}
% \caption{xxx.}
% \begin{tabular}{cccccccccc}\toprule
%  \multirow{2}*{Dataset}&\multirow{2}*{Method}  &\multicolumn{4}{c}{InstructBLIP} &\multicolumn{4}{c}{LLaVA 1.5} \\ \cmidrule(lr){3-6} \cmidrule(lr){7-10}
%  & &Accuracy &Precision &Recall &F1 &Accuracy &Precision &Recall &F1\\
%  \midrule
%   % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
%   \multirow{5}*{AMBER}& base& & & & & & & & \\
%   & VCD& & & & & & & & \\
%   & M3ID& & & & & & & & \\
%   & AVISC& & & & & & & & \\
%   & Octopus& & & & & & & & \\

  
% % \midrule
% % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% % \midrule
% \bottomrule
% \end{tabular}

% \label{tab:main}
% \end{table*}
\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
\caption{xxx.}
\begin{tabular}{ccccc}\toprule
 Method&Accuracy &Precision &Recall &F1\\
 \midrule
  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  LLaVA-v1.5-7B& 67.00  & 85.45  & 60.95  & 71.10 \\
  + VCD& 67.30  & 86.10  & 60.55  & 71.10  \\
  + M3ID& 67.25  & \textbf{86.50}  & 60.05  & 70.90  \\
  + AVISC& 70.70  & 85.45  & 67.55  & 75.45  \\
  + Octopus& \textbf{76.70}  & 82.00  & \textbf{83.40}  & \textbf{82.70}  \\
  \midrule
  InstructBLIP& 68.20  & 79.00  & 70.70  & 74.60 \\
  + VCD& 69.95  & 80.70  & 71.60  & 75.90  \\
  + M3ID& 69.05  & 79.70  & 71.25  & 75.25  \\
  + AVISC& 72.60  & 72.60  & 76.10  & 78.60  \\
  + Octopus& \textbf{74.00}  & \textbf{83.10}  & \textbf{76.60}  & \textbf{79.70}  \\

  
% \midrule
% \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% \midrule
\bottomrule
\end{tabular}

\label{tab:main}
\end{table}

==> no_use_fig_table/table_45.tex <==
\begin{table*}
\begin{minipage}{\textwidth}
\begin{minipage}[t]{0.48\textwidth}
\makeatletter\def\@captype{table}
\caption{xxx.}
\label{tab:table4}
\resizebox{1\textwidth}{!}{
\begin{tabular}{ccccccc}\toprule
 VCD&M3ID&AVISC&CHAIR $\downarrow$&Cover. $\uparrow$ &Hal. $\downarrow$&Cog. $\downarrow$\\
 \midrule
  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  % &&& 83.77  & 92.31  & 73.67  & 81.94 \\
  % \checkmark &&& 85.43  & 93.25  & 76.40  & 83.99 \\
  % & \checkmark && 86.13  & 92.59  & 73.33  & 81.85 \\
  % && \checkmark& 83.80  & 92.04  & 74.00  & 82.04 \\
  % \checkmark &\checkmark && 86.33  & 93.36  & 76.57  & 84.14 \\
  % \checkmark && \checkmark& 85.30  & 94.61  & 75.87  & 84.21 \\
  % & \checkmark &\checkmark & 86.27  & 94.86  & 75.00  & 83.78 \\
  % \checkmark &\checkmark &\checkmark & \textbf{86.53}  & \textbf{95.14}  & \textbf{77.00}  & \textbf{85.11} \\
  &&&   &   &  &  \\
  \checkmark &&& &   &  & \\
  & \checkmark && &   &  & \\
  && \checkmark& &   &  & \\
  \checkmark &\checkmark && &   &  & \\
  \checkmark && \checkmark& &   &  & \\
  & \checkmark &\checkmark & &   &  & \\
  \checkmark &\checkmark &\checkmark & &   &  & \\
  
 
  
% \midrule
% \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% \midrule
\bottomrule
\end{tabular}
}
\end{minipage}\hspace{10mm}
\begin{minipage}[t]{0.48\textwidth}
\makeatletter\def\@captype{table}
\caption{xxx.}
\label{tab:table5}
\resizebox{1\textwidth}{!}{
\begin{tabular}{lccccc}\toprule

  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  &Setting&CHAIR $\downarrow$&Cover. $\uparrow$ &Hal. $\downarrow$&Cog. $\downarrow$ \\
  \midrule
  \multirow{3}*{Controllability}&Cover.&&&& \\
  % &Hal.&&&& \\
  &CHAIR&&&& \\
  \midrule
  \multirow{3}*{RL Technologies}&Monte Carlo&&&& \\
  &PPO&&&& \\
  &DPO&&&& \\
  % \midrule
  % \multirow{3}*{Training quantity}&3000&&&& \\
  % &6000&&&& \\
  % &10000&&&& \\
 
  
% \midrule
% \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% \midrule
\bottomrule
\end{tabular}
}
\end{minipage}

\end{minipage}
\end{table*}


==> no_use_fig_table/table_fuluxiaorong.tex <==
\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
\caption{\textbf{Ablation study.} We selected different numbers of contrastive decoding methods as candidates to demonstrate the effectiveness of our approach. VCD~\cite{leng2024mitigating}, M3ID~\cite{favero2024multi} and AVISC~\cite{woo2024don} represent different comparative decoding methods.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccccccc}\toprule
 % VCD&M3ID&AVISC&CHAIR $\downarrow$&Cover. $\uparrow$ &Hal. $\downarrow$&Cog. $\downarrow$\\
 VCD&M3ID&AVISC&Accuracy &Precision &Recall &F1\\
 \midrule
  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  &&& 83.77  & 92.31  & 73.67  & 81.94 \\
  \checkmark &&& 85.43  & 93.25  & 76.40  & 83.99 \\
  & \checkmark && 86.13  & 92.59  & 73.33  & 81.85 \\
  && \checkmark& 84.67  & 97.88  & 70.87  & 82.21 \\
  \checkmark &\checkmark && 86.33  & 93.36  & 76.57  & 84.14 \\
  \checkmark && \checkmark& 85.30  & 94.61  & 75.87  & 84.21 \\
  & \checkmark &\checkmark & 86.27  & 94.86  & 75.00  & 83.78 \\
  % \checkmark &\checkmark &\checkmark & \textbf{86.53}  & \textbf{95.14}  & \textbf{77.00}  & \textbf{85.11} \\
  \checkmark &\checkmark &\checkmark & 86.53  & 95.14  & 77.00  & 85.11 \\
  % &&&  7.95  & 44.45  & 31.00  & 2.15  \\
  % \checkmark &&& 6.50  & 46.20  & 26.10  & 2.20 \\
  % & \checkmark && 6.70  & 46.50  & 27.80  & 1.95 \\
  % && \checkmark& 6.00  & 48.90  & 26.00  & 1.45 \\
  % \checkmark &\checkmark && 5.50  & 49.70  & 25.80  & 1.20 \\
  % \checkmark && \checkmark& 5.70  & 49.20  & 25.30  & 1.50 \\
  % & \checkmark &\checkmark & 5.50  & 49.40  & 26.20  & 1.60 \\
  % % \checkmark &\checkmark &\checkmark & \textbf{4.80}  & \textbf{49.20}  & \textbf{23.40}  & \textbf{1.20} \\
  % \checkmark &\checkmark &\checkmark & 4.80  & 49.20 & 23.40  & 1.20 \\
  
 
  
% \midrule
% \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% \midrule
\bottomrule
\end{tabular}
}

\label{tab:fuluxiaorong}
\end{table}

==> no_use_fig_table/table_pailie.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
\caption{xxx.}
\label{tab:pailie}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{ccc}\toprule

  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  {\#Candidate CDs}&& Combinations \\
  \midrule
  \multirow{3}*{One}&AVISC&[AVISC,AVISC,AVISC] \\
  % &Hal.&&&& \\
  &VCD&[VCD,VCD,VCD]\\
  &M3ID&[M3ID,M3ID,M3ID] \\
  \midrule
  \multirow{6}*{Two}&AVISC+VCD&{\makecell[c]{{[VCD, VCD, VCD], [VCD, VCD, AVISC],[VCD, AVISC, VCD],[AVISC, VCD, VCD], [AVISC, VCD, AVISC],} \\ {[VCD, AVISC, AVISC],[AVISC, AVISC, VCD], [AVISC, AVISC, AVISC]}}} \\ \cmidrule(lr){2-3}
  &VCD+M3ID&{\makecell[c]{{[M3ID, VCD, M3ID], [M3ID, VCD, VCD], [M3ID, M3ID, VCD],[M3ID, M3ID, M3ID],[VCD, M3ID, M3ID],}\\ {[VCD, M3ID, VCD],[VCD, VCD, M3ID], [VCD, VCD, VCD]}}}\\ \cmidrule(lr){2-3}
  &AVISC+M3ID&\makecell[c]{{[M3ID, AVISC, M3ID], [M3ID, AVISC, AVISC], [M3ID, M3ID, AVISC],[M3ID, M3ID, M3ID], [AVISC, M3ID, M3ID],}\\ {[AVISC, M3ID, AVISC], [AVISC, AVISC, M3ID], [AVISC, AVISC, AVISC]}} \\ 
  \midrule
  Three&AVISC+VCD+M3ID&\makecell[c]{{[AVISC, AVISC, AVISC], [AVISC, AVISC, VCD], [AVISC, AVISC, M3ID], [AVISC, VCD, AVISC], [AVISC, VCD, VCD],}\\ {[AVISC, VCD, M3ID], [AVISC, M3ID, AVISC], [AVISC, M3ID, VCD], [AVISC, M3ID, M3ID], [VCD, AVISC, AVISC],}\\ {[VCD, AVISC, VCD], [VCD, AVISC, M3ID], [VCD, VCD, AVISC], [VCD, VCD, VCD], [VCD, VCD, M3ID],} \\{[VCD, M3ID, AVISC], [VCD, M3ID, VCD], [VCD, M3ID, M3ID], [M3ID, AVISC, AVISC], [M3ID, AVISC, VCD],}\\ {[M3ID, AVISC, M3ID], [M3ID, VCD, AVISC], [M3ID, VCD, VCD], [M3ID, VCD, M3ID], [M3ID, M3ID, AVISC],}\\ {[M3ID, M3ID, VCD], [M3ID, M3ID, M3ID]}} \\
  
  % \midrule
  % \multirow{3}*{Training quantity}&3000&&&& \\
  % &6000&&&& \\
  % &10000&&&& \\
 
  
% \midrule
% \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% \midrule
\bottomrule
\end{tabular}
}
\end{table*}

==> table/tabel_popeother.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
\caption{Comparison with the state-of-the-art methods on the discriminative tasks. We evaluate the discriminative task on the GQA and A-OKVQA datasets and report the accuracy and F1 score. %$^\ddagger$ indicate the results from ~\cite{woo2024don}, and 
$^\dagger$ signifies results reproduced with the official implementation codes.}
\begin{tabular}{clcccccccc}\toprule
 % &\multicolumn{2}{c}{AMBER}&\multicolumn{8}{c}{POPE\_MSCOCO} \\ 
 % \cmidrule[0.4pt](lr){2-3} 
 % \cmidrule[0.4pt](lr){4-11}
 &&\multicolumn{2}{c}{Random}&\multicolumn{2}{c}{Popular}&\multicolumn{2}{c}{Adversarial}&\multicolumn{2}{c}{ALL}  \\
 \cmidrule[0.4pt](lr){3-4}
 \cmidrule[0.4pt](lr){5-6}
 \cmidrule[0.4pt](lr){7-8}
 \cmidrule[0.4pt](lr){9-10}
 % \cmidrule[0.4pt](lr){10-11}
 &&Accuracy &F1 &Accuracy &F1 &Accuracy &F1 &Accuracy &F1\\
 \midrule
  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  \multirow{10}*{A-OKVQA}&LLaVA-1.5\cite{liu2024improved}
  %$^\ddagger$
  & 84.93  & 84.07  & 80.90  & 80.64  & 74.80  & 75.59  & 80.21  & 80.10  \\
  &+VCD~\cite{leng2024mitigating}
  %$^\ddagger$ 
  & 85.53  & 85.12  & 81.17  & 81.46  & 75.03  & 76.72  & 80.58  & 81.10  \\
  % + LCD & - & -& 85.73  & 83.76  & 85.40  & 83.47  & 83.33 & 81.62  & -  & - \\
  % LLaVA-1.5+ICD&-  &- & 87.51& 83.28 & 83.15 & 83.91 & 79.13 & 80.41&-&-   \\
  % LLaVA-1.5+ConVis& - &- &84.70  &-   &83.2   &-   &81.1  &-  &83.00  &-   \\
  % LLaVA-1.5+OPERA& - &- &84.40  &-   &83.4   &-   &81.2  &-  &83.00  &-   \\
  % LLaVA-1.5+HALC& - &- &50.8  &-   &50.6   &-   &50.4  &-  &50.6  &-   \\
  &+M3ID~\cite{favero2024multi}
  $^\dagger$
  & 85.06  & 84.30  & 80.90  & 80.77  & 74.80  & 76.15  & 80.25  & 80.41  \\
  &+AVISC~\cite{woo2024don}
  %$^\ddagger$
  & 87.33  & 86.14  & 85.03  & 84.03  & 79.27  & 79.16  & 83.88  & 83.11   \\
  &+Octopus (ours)& \textbf{88.57}  & \textbf{88.05}  & \textbf{85.74}  & \textbf{85.92}  & \textbf{80.10}  & \textbf{80.23}  & \textbf{84.93}  & \textbf{84.77}  \\
    \cmidrule[0.4pt](lr){2-10}
  &InstructBLIP~\cite{10.5555/3666122.3668264}
  %$^\ddagger$
  & 81.33  & 82.21  & 76.87  & 78.82  & 71.40  & 74.96  & 76.53  & 78.66  \\
  % InstructBLIP+ICD&-&-&84.36& 83.82& 77.88& 78.70 & 75.17 & 77.23 &79.14  &79.92    \\
  &+ICD~\cite{wang2024mitigating}&85.82&86.29&81.64&83.32&74.42&78.48&80.63&82.70\\
  % InstructBLIP+OPERA& - & -&84.57& 83.74 & 78.24& 79.15 & 74.59 & 76.33 &79.13  &79.74   \\
  &+VCD~\cite{leng2024mitigating}
  %$^\ddagger$
  & 81.57  & 82.42  & 77.30  & 79.19  & 72.47  & 75.97  & 77.11  & 79.19  \\
  &+M3ID~\cite{favero2024multi}
  $^\dagger$
  & 82.37  & 82.70  & 78.33  & 79.55  & 72.07  & 74.94  & 77.59  & 79.06   \\
  &+AVISC~\cite{woo2024don}
  %$^\ddagger$
  & 87.10  & 86.62  & 82.47  & 82.65  & 76.47  & 78.03  & 82.01  & 82.43  \\
  &+Octopus (ours)&\textbf{87.43}  & \textbf{87.14}  & \textbf{83.13}  & \textbf{83.34}  & \textbf{77.20}  & \textbf{78.85}  & \textbf{82.61}  & \textbf{83.03}    \\
  \midrule
  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  \multirow{10}*{GQA}&LLaVA-1.5\cite{liu2024improved}
  %$^\ddagger$
  & 84.80  & 84.16  & 79.37  & 79.64  & 76.00  & 76.89  & 80.06  & 80.23 \\
  &+VCD~\cite{leng2024mitigating}
  %$^\ddagger$ 
  & 85.63  & 85.38  & 78.73  & 79.78  & 76.40  & 78.15  & 80.25  & 81.10  \\
  % + LCD & - & -& 85.73  & 83.76  & 85.40  & 83.47  & 83.33 & 81.62  & -  & - \\
  % LLaVA-1.5+ICD&-  &- & 87.51& 83.28 & 83.15 & 83.91 & 79.13 & 80.41&-&-   \\
  % LLaVA-1.5+ConVis& - &- &84.70  &-   &83.2   &-   &81.1  &-  &83.00  &-   \\
  % LLaVA-1.5+OPERA& - &- &84.40  &-   &83.4   &-   &81.2  &-  &83.00  &-   \\
  % LLaVA-1.5+HALC& - &- &50.8  &-   &50.6   &-   &50.4  &-  &50.6  &-   \\
  &+M3ID~\cite{favero2024multi}
  $^\dagger$
  & 84.80  & 84.23  & 79.23  & 79.63  & 75.83  & 76.93  & 79.95  & 80.26  \\
  &+AVISC~\cite{woo2024don}
  %$^\ddagger$
  & 87.40  & 86.21  & 83.33  & 82.54  & 80.37  & 80.00  & 83.70  & 82.92  \\
  &+Octopus (outs)& \textbf{88.79}  & \textbf{88.89}  & \textbf{84.23}  & \textbf{84.51}  & \textbf{81.79}  & \textbf{82.69}  & \textbf{84.78}  & \textbf{85.01}   \\
  \cmidrule[0.4pt](lr){2-10}
  &InstructBLIP~\cite{10.5555/3666122.3668264}
  %$^\ddagger$
  & 80.57  & 81.60  & 74.67  & 77.20  & 72.63  & 75.92  & 75.96  & 78.24  \\
  % InstructBLIP+ICD&-&-&84.36& 83.82& 77.88& 78.70 & 75.17 & 77.23 &79.14  &79.92    \\
  &+ICD~\cite{wang2024mitigating}&85.10&85.29&78.80&80.87&75.17&77.65&79.69&81.27\\
  % InstructBLIP+OPERA& - & -&84.57& 83.74 & 78.24& 79.15 & 74.59 & 76.33 &79.13  &79.74   \\
  &+VCD~\cite{leng2024mitigating}
  %$^\ddagger$
  & 81.73  & 82.55  & 74.63  & 77.30  & 71.93  & 75.32  & 76.10  & 78.39  \\
  &+M3ID~\cite{favero2024multi}
  $^\dagger$
  & 81.17  & 81.57  & 75.77  & 77.50  & 73.47  & 75.94  & 76.80  & 78.34  \\
  &+AVISC~\cite{woo2024don}
  %$^\ddagger$
  & 85.30  & 84.65  & 80.63  & 80.72  & 77.60  & 78.31  & 81.18  & 81.23  \\
  &+Octopus (ours)& \textbf{86.71}  & \textbf{86.10}  & \textbf{82.93}  & \textbf{82.51}  & \textbf{79.88}  & \textbf{79.20}  & \textbf{82.55}  & \textbf{82.92}   \\


% \midrule
% \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% \midrule
\bottomrule
\end{tabular}

\label{tab:pope_other}
\end{table*}


==> table/table_efficiency.tex <==
\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
\caption{Model efficiency analysis.}
\resizebox{0.28\textwidth}{!}{
\begin{tabular}{ccc}\toprule
 % VCD&M3ID&AVISC&CHAIR $\downarrow$&Cover. $\uparrow$ &Hal. $\downarrow$&Cog. $\downarrow$\\
 &FLOPs(G)&Parameters(M)\\
 \midrule
  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  % LLaVA&17227.6&7368.6\\
  % CD&34455.2&7368.6\\
  % Octopus&34455.4(0.001\%)&7540.7(2.3\%) \\
  LLaVA&9260.6&7368.6\\
  CD&18521.2&7368.6\\
  Octopus&18585.4(0.35\%)&7540.7(2.3\%) \\
  
  
 
  
% \midrule
% \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{AMBER}}} \\
% \midrule
\bottomrule
\end{tabular}
}

\label{tab:efficiency}
\end{table}

==> table/table_stability.tex <==
\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
\caption{Model stability analysis.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccccc}\toprule
 % VCD&M3ID&AVISC&CHAIR $\downarrow$&Cover. $\uparrow$ &Hal. $\downarrow$&Cog. $\downarrow$\\
 &CHAIR $\downarrow$&Cover. $\uparrow$ &Hal. $\downarrow$&Cog. $\downarrow$ \\
 \midrule
  % \rowcolor{lightgray} \multicolumn{11}{c}{\textbf{\textit{POPE}}} \\ \midrule
  
  1&4.8&49.2&23.4&1.2 \\
  2&4.6&48.6&24.0&0.9 \\
  3&4.4&47.7&22.8&1.0 \\
  4&5.0&48.2&23.9&1.4 \\
  5&5.1&49.9&24.1&1.3 \\
  Average&$4.78\pm0.07$&$48.72\pm0.59$&$23.64\pm0.23$&$1.16\pm0.03$ \\

\bottomrule
\end{tabular}
}

\label{tab:stability}
\end{table}
